Machine Learning Quantum States -- Extensions to Fermion-Boson Coupled Systems and Excited-State Calculations

To analyze quantum many-body Hamiltonians, recently, machine learning techniques have been shown to be quite useful and powerful. However, the applicability of such machine learning solvers is still limited. Here, we propose schemes that make it possible to apply machine learning techniques to analyze fermion-boson coupled Hamiltonians and to calculate excited states. As for the extension to fermion-boson coupled systems, we study the Holstein model as a representative of the fermion-boson coupled Hamiltonians. We show that the machine-learning solver achieves highly accurate ground-state energy, improving the accuracy substantially compared to that obtained by the variational Monte Carlo method. As for the calculations of excited states, we propose a different approach than that proposed in K. Choo et al., Phys. Rev. Lett. 121 (2018) 167204. We discuss the difference in detail and compare the accuracy of two methods using the one-dimensional $S=1/2$ Heisenberg chain. We also show the benchmark for the frustrated two-dimensional $S=1/2$ $J_1$-$J_2$ Heisenberg model and show an excellent agreement with the results obtained by the exact diagonalization. The extensions shown here open a way to analyze general quantum many-body problems using machine learning techniques.

==> 12345 <==
56c56
< The RBM can represent quantum states showing volume law entanglement entropy.~\cite{PhysRevX.7.021021,PhysRevB.97.085104} 
---
> The RBM can represent quantum states showing volume-law entanglement entropy.~\cite{PhysRevX.7.021021,PhysRevB.97.085104} 
62c62
< Several studies have introduced different neural network than the RBM~\cite{Gao_Ncom,PhysRevB.99.165123,DBM_NC,doi:10.1142/S0219749918400087,doi:10.7566/JPSJ.86.093001,doi:10.7566/JPSJ.87.014001,doi:10.7566/JPSJ.87.074002,PhysRevB.97.035116,PhysRevB.100.125124,Westerhout_arXiv}. 
---
> Several studies have introduced different neural network than the RBM~\cite{Gao_Ncom,PhysRevB.99.165123,DBM_NC,doi:10.1142/S0219749918400087,doi:10.7566/JPSJ.86.093001,doi:10.7566/JPSJ.87.014001,doi:10.7566/JPSJ.87.074002,PhysRevB.97.035116,PhysRevB.100.125124,Westerhout_2020}. 
65c65
< frustrated spin systems~\cite{PhysRevB.97.035116,PhysRevB.98.104426,PhysRevB.100.125124,PhysRevB.100.125131,Westerhout_arXiv},
---
> frustrated spin systems~\cite{PhysRevB.97.035116,PhysRevB.98.104426,PhysRevB.100.125124,PhysRevB.100.125131,Westerhout_2020},
69c69
< excited states~\cite{PhysRevLett.121.167204,Vieijra_arXiv},
---
> excited states~\cite{PhysRevLett.121.167204,Vieijra_2020},
72c72
< quantum states with nonabelian or anyonic symmetries~\cite{Vieijra_arXiv}. 
---
> quantum states with nonabelian or anyonic symmetries~\cite{Vieijra_2020}. 
121c121
< For the latter use, it is convenient to define occupation and dimensionless displacement operators ($\hat{n}^{\rm s}_i$ and $\hat{x}^{\rm s}_i $, respectively) in a staggered way: 
---
> For later use, it is convenient to define occupation and dimensionless displacement operators ($\hat{n}^{\rm s}_i$ and $\hat{x}^{\rm s}_i $, respectively) in a staggered way: 
206c206
< \includegraphics[width=0.42\textwidth]{phonon_basis.eps}
---
> \includegraphics[width=0.42\textwidth]{69575_Fig1.eps}
207a208
> (Color online)
231c232
< In the actual calculations, we impose translational symmetry, and the number is reduced to $2 (m_{\rm max} \! +\! 1)$.
---
> In the actual calculations, we impose the translational symmetry, and the number is reduced to $2 (m_{\rm max} \! +\! 1)$.
275c276
< \includegraphics[width=0.42\textwidth]{structure_RBM.eps}
---
> \includegraphics[width=0.42\textwidth]{69575_Fig2.eps}
276a278
> (Color online)
303c305
< \includegraphics[width=0.42\textwidth]{definition_sigma.eps}
---
> \includegraphics[width=0.42\textwidth]{69575_Fig3.eps}
304a307
> (Color online)
306a310
> In this example, three visible units are introduced to represent phonon configurations.
316c320
< we prepare one visible unit for electron configuration and $M$ visible units for phonon configuration for each site. 
---
> we prepare one visible unit for electron configuration and $M$ visible units for phonon configuration for each site (see Fig.~\ref{fig_definition_sigma}). 
354c358,359
< Following the previous study, we use periodic (anti-periodic) boundary condition when the number of electrons is odd (even). 
---
> Following the previous studies~\cite{PhysRevB.53.9676,PhysRevB.89.195139}, 
> we use periodic (anti-periodic) boundary condition when the number of electrons is odd (even). 
367c372
< \includegraphics[width=0.9\textwidth]{1D_Holstein_ene.eps}
---
> \includegraphics[width=0.9\textwidth]{69575_Fig4.eps}
368a374
> (Color online)
406c412
< In the present Hamiltonian, the charge-charge correlation function has a peak at the momentum ${\bf q} = \pi$, and the charge structure factor is given by 
---
> In the present Hamiltonian, the charge-charge correlation function has a peak at the momentum $ q = \pi$, and the charge structure factor is given by 
415c421
< \includegraphics[width=0.45\textwidth]{1D_Holstein_Sc.eps}
---
> \includegraphics[width=0.45\textwidth]{69575_Fig5.eps}
416a423
> (Color online)
426a434
> We employ the periodic boundary condition to compare our results with those of Ref. ~\citen{FEHSKE2005699}.
597c605
< \includegraphics[width=0.48\textwidth]{1D_Heis_ene.eps}
---
> \includegraphics[width=0.48\textwidth]{69575_Fig6.eps}
598a607
> (Color online)
665c674
< \includegraphics[width=0.45\textwidth]{2D_J1J2_ene.eps}
---
> \includegraphics[width=0.45\textwidth]{69575_Fig7.eps}
666a676
> (Color online)
695c705
< As is discussed in Ref.~\citen{PhysRevB.96.205152}, by combining the RBM with other powerful wave functions, the same accuracy can be achieved by smaller number of variational parameters.  
---
> As is discussed in Ref.~\citen{PhysRevB.96.205152}, by combining the RBM with other powerful wave functions, the same accuracy would be achieved by smaller number of variational parameters.  
698d707
< 
736a746
> 
740a751,753
> 
> 
> 

